Performance Analysis of Semi-Persistent Scheduling Throughput in 5G NR-V2X: A MAC Perspective

The packet throughput in 5th Generation (5G) New Radio (NR) Vehicle-to-Everything (V2X) is highly dependent on the Medium Access Control (MAC) based scheduling algorithm with no base station participation. In particular, the Semi-Persistent Scheduling (SPS) algorithm has been standardized by the 3rd Generation Partnership Project (3GPP) for V2X resource scheduling in the out-of-coverage scenario. This paper analyzes the NR-V2X SPS throughput from the MAC perspective, where the packet reception ratio (PRR) and half-duplex (HD) effect dominate. We first investigate the average throughput in the fully connected vehicular network, in which all the vehicles share the same throughput. Subsequently, the average throughput as a function of distance in the partially connected vehicular network is analyzed. The Monte Carlo simulation results show that increasing the resource keeping probability can improve the average throughput. Meanwhile, in the partially connected network, the lower resource keeping probability is prone to obtaining the higher throughput gain by increasing the number of subchannels.

==> tmp.tex <==
\section{Demos}

%figures:
% Double column:
\begin{figure*}[t]
    \centering
    \includegraphics[width = .8\textwidth]{tier.png}
    \caption{Illustration of three-tier structure: AP $1$ selects two 20 MHz sub-channels in 2.4 GHz band, two 20 MHz sub-channels in 5 GHz band, and a 20 MHz channel in 6 GHz based on a certain policy $\pi$. Then AP $1$ allocates these $5$ resource units to its attached stations.}
    \label{fig:tier}
\end{figure*}

%normal:
\begin{figure}[t]
    \centering
    \includegraphics[width=.43\textwidth]{Performance.eps}
    \caption{Average throughput comparison.}
    \label{fig:performance}
\end{figure}

%multi figures
\begin{figure}[htbp] 
  \centering
  \subfigure[Total utility vs the number of URLLC user numbers per Mini-slot. ] {\includegraphics[width=.4\textwidth]{max_rate.eps}}\quad
  \subfigure[ The $\frac{\Phi(n)}{DRC(n)}$ of each eMBB user, $M = 8$ per mini-slot.] {\includegraphics[width=.4\textwidth]{mr_fair.eps}}
  \caption{Simulation result with the objective of maximizing total rate, i.e., $U(\Phi(n)) = \Phi(n)$.}
  \label{fig:mr}
\end{figure}
